Optimizing Hyperparameters with Conformal Quantile Regression

Many state-of-the-art hyperparameter optimization (HPO) algorithms rely on model-based optimizers that learn surrogate models of the target function to guide the search. Gaussian processes are the de facto surrogate model due to their ability to capture uncertainty but they make strong assumptions about the observation noise, which might not be warranted in practice. In this work, we propose to leverage conformalized quantile regression which makes minimal assumptions about the observation noise and, as a result, models the target function in a more realistic and robust fashion which translates to quicker HPO convergence on empirical benchmarks. To apply our method in a multi-fidelity setting, we propose a simple, yet effective, technique that aggregates observed results across different resource levels and outperforms conventional methods across many empirical tasks.

==> figures/all/tab1.tex <==
\begin{tabular}{l|rrrrrr|rrrrr}
\toprule
 & \RS{} & \TPE{} & \REA{} & \GP{} & \BORE{} & \CQR{} & \ASHA{} & \BOHB{} & \MOB{} & \HT{} & \CQRMF{} \\
benchmark &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
fcnet-0 & 9.66 & 8.12 & 4.64 & 5.26 & 4.20 & \textbf{3.43} & 8.30 & 7.84 & 5.21 & 5.03 & \textbf{4.31} \\
fcnet-1 & 9.77 & 9.61 & 7.45 & 5.52 & 6.82 & \textbf{4.82} & 6.20 & 6.35 & \textbf{2.96} & 3.14 & 3.34 \\
fcnet-2 & 9.06 & 8.70 & 7.09 & 7.30 & \textbf{6.05} & 6.86 & 4.79 & 4.41 & 3.79 & 4.31 & \textbf{3.65} \\
fcnet-3 & 9.81 & 9.02 & 5.68 & 5.79 & \textbf{3.74} & 5.01 & 6.62 & 6.54 & 4.55 & \textbf{3.95} & 5.29 \\
lcbench-0 & 5.46 & 6.57 & 6.96 & \textbf{5.11} & 5.12 & 5.49 & 5.00 & \textbf{4.89} & 7.02 & 7.91 & 6.48 \\
lcbench-1 & 9.12 & 8.58 & 7.76 & 6.72 & \textbf{5.56} & 5.76 & 3.91 & 4.00 & 4.76 & 6.17 & \textbf{3.65} \\
lcbench-2 & 8.57 & 8.20 & 8.02 & 6.71 & 6.65 & \textbf{5.81} & 3.81 & \textbf{3.67} & 5.29 & 5.53 & 3.74 \\
lcbench-3 & 8.97 & 8.80 & 7.93 & 5.97 & 5.90 & \textbf{5.03} & 4.97 & 4.45 & 5.25 & 5.18 & \textbf{3.54} \\
lcbench-4 & 8.48 & 8.34 & 8.81 & 7.18 & 6.59 & \textbf{6.12} & 3.86 & 3.84 & 4.90 & 5.16 & \textbf{2.73} \\
nas201-0 & 8.22 & 8.18 & 8.16 & 7.21 & 7.80 & \textbf{6.98} & 4.22 & 4.12 & \textbf{3.25} & 3.52 & 4.33 \\
nas201-1 & 8.17 & 8.06 & 8.16 & 7.43 & 7.58 & \textbf{6.94} & 4.41 & 4.55 & 3.56 & \textbf{3.24} & 3.91 \\
nas201-2 & 8.01 & 7.80 & 8.02 & 7.76 & 7.71 & \textbf{6.92} & 3.96 & 4.47 & 3.65 & \textbf{3.64} & 4.04 \\
yahpo-0 & 8.96 & 8.89 & \textbf{4.32} & 8.51 & 6.63 & 7.08 & 5.06 & 5.33 & 3.63 & 4.77 & \textbf{2.82} \\
Average & 8.64 & 8.38 & 7.16 & 6.65 & 6.18 & \textbf{5.87} & 5.01 & 4.96 & 4.45 & 4.73 & \textbf{3.99} \\
\bottomrule
\end{tabular}


==> figures/multi-fidelity-extension/tab1.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
 & \ASHA{} & \MOB{} & \REAMF{} & \GPMF{} & \BOREMF{} & \QRMF{} & \CQRMF{} \\
benchmark &  &  &  &  &  &  &  \\
\midrule
fcnet-0 & 5.84 & 3.74 & 3.28 & 5.48 & \textbf{\textbf{2.62}} & 3.96 & 3.08 \\
fcnet-1 & 5.61 & \textbf{\textbf{2.84}} & 3.80 & 5.16 & 3.27 & 4.29 & 3.03 \\
fcnet-2 & 4.29 & \textbf{\textbf{3.28}} & 4.31 & 3.87 & 4.04 & 4.73 & 3.48 \\
fcnet-3 & 5.00 & 3.63 & \textbf{\textbf{2.86}} & 4.73 & 3.28 & 4.47 & 4.04 \\
lcbench-0 & \textbf{\textbf{3.07}} & 4.49 & 4.64 & 3.13 & 4.03 & 4.46 & 4.16 \\
lcbench-1 & 3.83 & 4.34 & 4.41 & 4.01 & 3.98 & 4.09 & \textbf{\textbf{3.34}} \\
lcbench-2 & 3.81 & 4.53 & 5.04 & 3.68 & \textbf{\textbf{3.40}} & 4.07 & 3.47 \\
lcbench-3 & 4.31 & 4.47 & 5.38 & 4.11 & 3.21 & 3.33 & \textbf{\textbf{3.19}} \\
lcbench-4 & 3.82 & 4.67 & 5.22 & 3.83 & 4.00 & 3.64 & \textbf{\textbf{2.82}} \\
nas201-0 & 4.12 & \textbf{\textbf{3.04}} & 3.39 & 4.25 & 4.38 & 4.86 & 3.95 \\
nas201-1 & 4.53 & \textbf{\textbf{3.48}} & 3.75 & 4.54 & 3.77 & 4.32 & 3.60 \\
nas201-2 & 3.79 & \textbf{\textbf{3.33}} & 4.25 & 3.93 & 4.30 & 4.83 & 3.58 \\
yahpo-0 & 5.08 & 4.09 & \textbf{\textbf{3.24}} & 5.15 & 3.25 & 3.90 & 3.28 \\
Average & 4.39 & 3.84 & 4.12 & 4.30 & 3.66 & 4.23 & \textbf{\textbf{3.46}} \\
\bottomrule
\end{tabular}


==> figures/multi-fidelity/tab1.tex <==
\begin{tabular}{lrrrrr}
\toprule
 & \ASHA{} & \BOHB{} & \MOB{} & \HT{} & \CQRMF{} \\
benchmark &  &  &  &  &  \\
\midrule
fcnet-0 & 4.12 & 3.90 & 2.50 & 2.39 & \textbf{\textbf{2.08}} \\
fcnet-1 & 4.04 & 4.09 & \textbf{\textbf{2.21}} & 2.30 & 2.36 \\
fcnet-2 & 3.36 & 3.18 & 2.70 & 3.07 & \textbf{\textbf{2.69}} \\
fcnet-3 & 3.67 & 3.61 & 2.61 & \textbf{\textbf{2.19}} & 2.93 \\
lcbench-0 & 2.40 & \textbf{\textbf{2.34}} & 3.30 & 3.85 & 3.10 \\
lcbench-1 & 2.75 & 2.81 & 3.11 & 3.88 & \textbf{\textbf{2.44}} \\
lcbench-2 & 2.83 & 2.69 & 3.41 & 3.54 & \textbf{\textbf{2.53}} \\
lcbench-3 & 3.16 & 2.98 & 3.29 & 3.16 & \textbf{\textbf{2.41}} \\
lcbench-4 & 2.81 & 2.93 & 3.46 & 3.65 & \textbf{\textbf{2.15}} \\
nas201-0 & 3.34 & 3.22 & \textbf{\textbf{2.53}} & 2.71 & 3.20 \\
nas201-1 & 3.42 & 3.31 & 2.78 & \textbf{\textbf{2.49}} & 3.00 \\
nas201-2 & 3.11 & 3.28 & 2.82 & \textbf{\textbf{2.75}} & 3.05 \\
yahpo-0 & 3.49 & 3.63 & 2.60 & 3.27 & \textbf{\textbf{2.01}} \\
Average & 3.27 & 3.23 & 2.87 & 3.02 & \textbf{\textbf{2.61}} \\
\bottomrule
\end{tabular}


==> figures/single-fidelity/tab1.tex <==
\begin{tabular}{lrrrrrr}
\toprule
 & \RS{} & \TPE{} & \REA{} & \GP{} & \BORE{} & \CQR{} \\
benchmark &  &  &  &  &  &  \\
\midrule
fcnet-0 & 5.39 & 4.60 & 2.90 & 3.18 & 2.68 & \textbf{\textbf{2.25}} \\
fcnet-1 & 5.01 & 4.84 & 3.40 & 2.53 & 3.15 & \textbf{\textbf{2.07}} \\
fcnet-2 & 4.32 & 4.11 & 3.31 & 3.42 & \textbf{\textbf{2.73}} & 3.11 \\
fcnet-3 & 5.27 & 4.72 & 3.15 & 3.00 & \textbf{\textbf{2.09}} & 2.76 \\
lcbench-0 & 3.36 & 3.93 & 4.13 & 3.15 & \textbf{\textbf{3.12}} & 3.30 \\
lcbench-1 & 4.65 & 4.26 & 3.90 & 3.09 & \textbf{\textbf{2.47}} & 2.63 \\
lcbench-2 & 4.32 & 4.12 & 3.86 & 3.09 & 2.99 & \textbf{\textbf{2.62}} \\
lcbench-3 & 4.52 & 4.46 & 4.00 & 2.87 & 2.80 & \textbf{\textbf{2.34}} \\
lcbench-4 & 3.98 & 4.03 & 4.34 & 3.08 & 2.87 & \textbf{\textbf{2.70}} \\
nas201-0 & 3.78 & 3.74 & 3.77 & 3.20 & 3.58 & \textbf{\textbf{2.94}} \\
nas201-1 & 3.72 & 3.68 & 3.83 & 3.25 & 3.46 & \textbf{\textbf{3.06}} \\
nas201-2 & 3.72 & 3.59 & 3.75 & 3.45 & 3.57 & \textbf{\textbf{2.93}} \\
yahpo-0 & 4.47 & 4.32 & \textbf{\textbf{2.17}} & 4.08 & 2.82 & 3.15 \\
Average & 4.35 & 4.18 & 3.58 & 3.18 & 2.95 & \textbf{\textbf{2.76}} \\
\bottomrule
\end{tabular}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> results/tab1.tex <==
\begin{tabular}{l|rrrrrr|rrrrr}
\toprule
 & \RS{} & \REA{} & \TPE{} & \GP{} & \BORE{} & \QR{} & \ASHA{} & \BOHB{} & \MOB{} & \XGBlastnocache{} & \QRMF{} \\
benchmark &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
\FCNet{} & 0.85 & 0.61 & 0.75 & 0.42 & 0.42 & \textbf{0.37} & 0.55 & 0.53 & 0.41 & \textbf{0.29} & 0.29 \\
\LCBench{} & 0.69 & 0.74 & 0.63 & 0.47 & \textbf{0.45} & 0.47 & 0.45 & 0.40 & 0.49 & \textbf{0.31} & 0.32 \\
\NASBench{} & 0.75 & 0.70 & 0.74 & 0.66 & \textbf{0.52} & 0.55 & 0.35 & 0.35 & 0.31 & \textbf{0.29} & 0.30 \\
\NASSurr{} & 0.76 & \textbf{0.42} & 0.76 & 0.72 & 0.46 & 0.54 & 0.39 & 0.42 & 0.30 & 0.27 & \textbf{0.24} \\
Average & 0.76 & 0.62 & 0.72 & 0.57 & \textbf{0.46} & 0.48 & 0.43 & 0.42 & 0.38 & 0.29 & \textbf{0.29} \\
\bottomrule
\end{tabular}

